Taming the Tail: NoI Topology Synthesis for Mixed DL Workloads on Chiplet-Based Accelerators

Heterogeneous chiplet-based systems improve scaling by disag-gregating CPUs/GPUs and emerging technologies (HBM/DRAM).However this on-package disaggregation introduces a latency inNetwork-on-Interposer(NoI). We observe that in modern large-modelinference, parameters and activations routinely move backand forth from HBM/DRAM, injecting large, bursty flows into theinterposer. These memory-driven transfers inflate tail latency andviolate Service Level Agreements (SLAs) across k-ary n-cube base-line NoI topologies. To address this gap we introduce an InterferenceScore (IS) that quantifies worst-case slowdown under contention.We then formulate NoI synthesis as a multi-objective optimization(MOO) problem. We develop PARL (Partition-Aware ReinforcementLearner), a topology generator that balances throughput, latency,and power. PARL-generated topologies reduce contention at the memory cut, meet SLAs, and cut worst-case slowdown to 1.2 times while maintaining competitive mean throughput relative to link-rich meshes. Overall, this reframes NoI design for heterogeneouschiplet accelerators with workload-aware objectives.

==> review_response.tex <==
REVIEW: Evaluation sections mostly restate plots instead of explaining why the results occur.
RESPONSE: Ok I need to add why such results occur although, I have explained at places in paper why such degredation happens and rationale behind them. need a consistent “why” sentence (or two) per key figure/panel

REVIEW: Insufficient details about the main contributions and RL formulation:
Missing clarity on the RL model, reward structure, and objectives.
Need to explain each term in the multi-objective loss (IS, latency, power, etc.), whether they are normalized, and what each weight (α₁–α₄) does.

RESPONSE:
1. I think state, action and reward is clearly mentioned in the paper im not sure what else they sxpect, would bellman equations help?
2. I have already mentioned that each term is extracted from api of simmulation tools like rapidchiplet
3. I have mentioned alphas are convex combos

so i must explain what the network/policy is, what ranges/normalization each term has before weighting, and what α’s do to the tradeoff

REVIEW: Need to include IS values of RL-generated topology in Figure 3. Add conclusions at the end of subsections (e.g., Section 2.2, 2.3).

RESPONSE: OK will add

REVIEW: The proofs of Claim A and Lemmas are not rigorous enough—they read more like intuitive reasoning than formal proofs.
Reviewers want cleaner theorem/lemma structure and clarity about assumptions.

RESPONSE: agreed, I must do this. I plan to look at other papers and books related and see how they rigourously present the proofs. 

REVIEW: The connection between the theory and experiments is underdeveloped:
The flow between the analytical model (Section 3) and empirical evaluation (Section 4) is unclear.
Need to explicitly show how the theoretical predictions (e.g., Kingman, min-cut bounds) motivate the design of the RL or relate to observed tail latency.

RESPOONSE: Ok I should add this but then problem is 4.5 page limit, but i can add couple of bridging lines per section + a short “theory→design→result” callout.

REVIEW: Lemma 2 assumption: independence between tokens may not hold in practice for real MoE routing, where gating decisions are correlated.

RESPONSE: needs to be crosschecked. but how does this changes things, can we have a more general case? why is independence needed? or can we prove this for both independent and dependent case.

REVIEW: Equation (2):
Metrics like IS, latency, power have different scales — unclear if they’re normalized before combining.
Missing discussion of physical constraints (area, routing, thermal) in the objective.

RESPONSE: I currently do not model all these physical constraints, this would require re writing the reward function and then introducing an upper bound on exploration of the agent(rl algorithm).


REVIEW: The RL formulation is under-described:
Missing architecture details (policy network, state/action definition, reward shaping).
No ablation study on the weights (α₁–α₄) or the IS term — unclear which part contributes most to the performance.

RESPONSE: agreed but then page limit. I can add training curves, bellman equations, i have mentioned that i have used maskedppo algo where i can add more detials about my model network. add one-paragraph architecture summary and tiny ablation

REVIEW: The evaluation lacks diversity and depth:
Only one workload family tested — Mixture-of-Experts (MoE).
No analysis on other sparse or irregular workloads (e.g., pruned LLMs, sparse HPC/scientific apps).
No discussion on how well the learned topology generalizes to unseen or different workloads.

RESPONSE: I can do this for future submission, tough for cam ready deadline and also limited space as its a workshop paper. Ill explicitly state scope and generalization limits in one line in Conclusion/Limitations

REVIEW: Scalability concerns:
RL-based search may struggle for larger node counts, as the search space grows combinatorially.
Framework not dynamic or hierarchical — potential scalability bottleneck for future systems.

RESPONSE: I do mention convergence issues of the RL. I also mentioned that the action space blow up had stunted the training in order to fix that i used maskable ppo algo and grid-pitch ablation which i did, further scalability needs to be verified.

REVIEW: “What specific property of the topology explains each result?”

RESPONSE: will add this

REVIEW: Missing rationale behind observed performance trends

RESPONSE: Need to explain reasons for residual latency or throughput loss.
Highlight which aspects of the learned topology help (shorter diameter, higher path multiplicity, better isolation, etc.).

REVIEW: Lack of discussion of real-world implementation constraints:
Port count, routing feasibility, signal integrity, and heat dissipation challenges of irregular topologies.
No mention of packaging-level constraints or physical design back-of-envelope (e.g., interposer wire lengths, energy/area).
Scalability and feasibility under real packaging limits remain open.

RESPONSE: I had tried to keep the env for rl as practical by adopting MI300 as closely as possible as possible but some choices were limited due to simulator capabilities.


